The Diversity and Scale Matter: Ubiquitous Transportation Mode Detection using Single Cell Tower Information

Detecting the transportation mode of a user is important for a wide range of applications. While a number of recent systems addressed the transportation mode detection problem using the ubiquitous mobile phones, these studies either leverage GPS, the inertial sensors, and/or multiple cell towers information. However, these different phone sensors have high energy consumption, limited to a small subset of phones (e.g. high-end phones or phones that support neighbouring cell tower information), cannot work in certain areas (e.g. inside tunnels for GPS), and/or work only from the user side. In this paper, we present a transportation mode detection system, MonoSense, that leverages the phone serving cell information only. The basic idea is that the phone speed can be correlated with features extracted from both the serving cell tower ID and the received signal strength from it. To achieve high detection accuracy with this limited information, MonoSense leverages diversity along multiple axes to extract novel features. Specifically, MonoSense extracts features from both the time and frequency domain information available from the serving cell tower over different sliding widow sizes. More importantly, we show also that both the logarithmic and linear RSS scales can provide different information about the movement of a phone, further enriching the feature space and leading to higher accuracy. Evaluation of MonoSense using 135 hours of cellular traces covering 485 km and collected by four users using different Android phones shows that it can achieve an average precision and recall of 89.26% and 89.84% respectively in differentiating between the stationary, walking, and driving modes using only the serving cell tower information, highlighting MonoSense ability to enable a wide set of intelligent transportation applications.

==> Collection <==
@incollection{Sohn06,
  title={Mobility detection using everyday {GSM} traces},
  author={Sohn, Timothy and Varshavsky, Alex and LaMarca, Anthony and Chen, Mike Y and Choudhury, Tanzeem and Smith, Ian and Consolvo, Sunny and Hightower, Jeffrey and Griswold, William G and De Lara, Eyal},
  booktitle={UbiComp 2006: Ubiquitous Computing},
  pages={212--224},
  year={2006},
  publisher={Springer}
},
@article{Traveltimeestimationonthesanfranciscobayareanetworkusingcellularphonesasprobes,
  title={Travel time estimation on the san francisco bay area network using cellular phones as probes},
  author={Ygnace, Jean-Luc and Drane, Chris and Yim, YB and De Lacvivier, Renaud},
  journal={California Partners for Advanced Transit and Highways (PATH)},
  year={2000}
},
@incollection{AccurateGSMindoorlocalization,
  title={Accurate GSM indoor localization},
  author={Otsason, Veljo and Varshavsky, Alex and LaMarca, Anthony and De Lara, Eyal},
  booktitle={UbiComp 2005: Ubiquitous Computing},
  pages={141--158},
  year={2005},
  publisher={Springer}
},
@book{Roadtrafficinformationfromcellularnetworksignaling,
  title={Road traffic information from cellular network signaling},
  author={Valerio, Danilo},
  year={2009},
  publisher={na}
},
@article{RouteChoiceEstimationBasedonCellularSignalingData,
  title={Route Choice Estimation Based on Cellular Signaling Data},
  author={Tettamanti, Tam{\'a}s and Demeter, Hunor and Varga, Istv{\'a}n},
  journal={Acta Polytechnica Hungarica},
  volume={9},
  number={4},
  pages={207--220},
  year={2012}
},
@inproceedings{stenneth11,
  title={Transportation mode detection using mobile phones and {GIS} information},
  author={Stenneth, Leon and Wolfson, Ouri and Yu, Philip S and Xu, Bo},
  booktitle={Proceedings of the 19th ACM SIGSPATIAL International Conference on Advances in Geographic Information Systems},
  pages={54--63},
  year={2011},
  organization={ACM}
},
@article{Recognizinghumanactivitiesuserindependentlyonsmartphonesbasedonaccelerometerdata,
  title={Recognizing human activities user-independently on smartphones based on accelerometer data},
  author={Siirtola, Pekka and R{\"o}ning, Juha},
  journal={International Journal of Interactive Multimedia and Artificial Intelligence},
  volume={1},
  number={5},
  year={2012}
},
@article{Reddy10,
  title={Using mobile phones to determine transportation modes},
  author={Reddy, Sasank and Mun, Min and Burke, Jeff and Estrin, Deborah and Hansen, Mark and Srivastava, Mani},
  journal={ACM Transactions on Sensor Networks (TOSN)},
  volume={6},
  number={2},
  pages={13},
  year={2010},
  publisher={ACM}
},
@inproceedings{ParsimoniousmobilityclassificationusingGSMandWiFitraces,
  title={Parsimonious mobility classification using GSM and WiFi traces},
  author={Mun, M and Estrin, Deborah and Burke, Jeff and Hansen, Mark},
  booktitle={Proceedings of the Fifth Workshop on Embedded Networked Sensors (HotEmNets)},
  year={2008}
},
@inproceedings{Nericellrichmonitoringofroadandtrafficconditionsusingmobilesmartphones,
  title={Nericell: rich monitoring of road and traffic conditions using mobile smartphones},
  author={Mohan, Prashanth and Padmanabhan, Venkata N and Ramjee, Ramachandran},
  booktitle={Proceedings of the 6th ACM conference on Embedded network sensor systems},
  pages={323--336},
  year={2008},
  organization={ACM}
},
@article{Activityrecognitionusingcellphoneaccelerometers,
  title={Activity recognition using cell phone accelerometers},
  author={Kwapisz, Jennifer R and Weiss, Gary M and Moore, Samuel A},
  journal={ACM SigKDD Explorations Newsletter},
  volume={12},
  number={2},
  pages={74--82},
  year={2011},
  publisher={ACM}
},
@inproceedings{Accelerometerbasedtransportationmodedetectiononsmartphones,
  title={Accelerometer-based transportation mode detection on smartphones},
  author={Hemminki, Samuli and Nurmi, Petteri and Tarkoma, Sasu},
  booktitle={Proceedings of the 11th ACM Conference on Embedded Networked Sensor Systems},
  pages={13},
  year={2013},
  organization={ACM}
},
@inproceedings{wang2010,
  title={Accelerometer based transportation mode recognition on mobile phones},
  author={Wang, Shuangquan and Chen, Canfeng and Ma, Jian},
  booktitle={Wearable Computing Systems (APWCS), 2010 Asia-Pacific Conference on},
  pages={44--46},
  year={2010},
  organization={IEEE}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Earlier Approches for activity recognaion %%%%%%%%%%%%%%%%
,
@incollection{bao2004activity,
  title={Activity recognition from user-annotated acceleration data},
  author={Bao, Ling and Intille, Stephen S},
  booktitle={Pervasive computing},
  pages={1--17},
  year={2004},
  publisher={Springer}
},
@inproceedings{ravi2005activity,
  title={Activity recognition from accelerometer data},
  author={Ravi, Nishkam and Dandekar, Nikhil and Mysore, Preetham and Littman, Michael L},
  booktitle={AAAI},
  volume={5},
  pages={1541--1546},
  year={2005}
},
@inproceedings{froehlich2009ubigreen,
  title={UbiGreen: investigating a mobile tool for tracking and supporting green transportation habits},
  author={Froehlich, Jon and Dillahunt, Tawanna and Klasnja, Predrag and Mankoff, Jennifer and Consolvo, Sunny and Harrison, Beverly and Landay, James A},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1043--1052},
  year={2009},
  organization={ACM}
},
@article{kang2005extracting,
  title={Extracting places from traces of locations},
  author={Kang, Jong Hee and Welbourne, William and Stewart, Benjamin and Borriello, Gaetano},
  journal={ACM SIGMOBILE Mobile Computing and Communications Review},
  volume={9},
  number={3},
  pages={58--68},
  year={2005},
  publisher={ACM}
},
@misc{alizadeh2009estimation,
  title={Estimation of speed and direction of travel in a WLAN positioning system using multiple position estimations},
  author={Alizadeh-Shabdiz, Farshid and Morgan, Edward J and Pahlavan, Kaveh},
  year={2009},
  month=jun # "~23",
  publisher={Google Patents},
  note={US Patent 7,551,929}
},
@misc{alizadeh2010estimation,
  title={Estimation of speed and direction of travel in a WLAN positioning system},
  author={Alizadeh-Shabdiz, Farshid and Morgan, Edward J and Pahlavan, Kaveh},
  year={2010},
  month=nov # "~16",
  publisher={Google Patents},
  note={US Patent 7,835,754}
},
@incollection{lamarca2005place,
  title={Place lab: Device positioning using radio beacons in the wild},
  author={LaMarca, Anthony and Chawathe, Yatin and Consolvo, Sunny and Hightower, Jeffrey and Smith, Ian and Scott, James and Sohn, Timothy and Howard, James and Hughes, Jeff and Potter, Fred and others},
  booktitle={Pervasive computing},
  pages={116--133},
  year={2005},
  publisher={Springer}
},
@inproceedings{mun2009peir,
  title={{PEIR}, the personal environmental impact report, as a platform for participatory sensing systems research},
  author={Mun, Min and Reddy, Sasank and Shilton, Katie and Yau, Nathan and Burke, Jeff and Estrin, Deborah and Hansen, Mark and Howard, Eric and West, Ruth and Boda},
  booktitle={Proceedings of the 7th international conference on Mobile systems, applications, and services},
  pages={55--68},
  year={2009},
  organization={ACM}
},
@inproceedings{patterson2003inferring,
  title={Inferring high-level behavior from low-level sensors},
  author={Patterson, Donald J and Liao, Lin and Fox, Dieter and Kautz, Henry},
  booktitle={UbiComp 2003: Ubiquitous Computing},
  pages={73--89},
  year={2003},
  organization={Springer}
},
@article{liao2007learning,
  title={Learning and inferring transportation routines},
  author={Liao, Lin and Patterson, Donald J and Fox, Dieter and Kautz, Henry},
  journal={Artificial Intelligence},
  volume={171},
  number={5},
  pages={311--331},
  year={2007},
  publisher={Elsevier}
},
@article{liao2007extracting,
  title={Extracting places and activities from {GPS} traces using hierarchical conditional random fields},
  author={Liao, Lin and Fox, Dieter and Kautz, Henry},
  journal={The International Journal of Robotics Research},
  volume={26},
  number={1},
  pages={119--134},
  year={2007},
  publisher={SAGE Publications}
},
@phdthesis{liao2006location,
  title={Location-based activity recognition},
  author={Liao, Lin},
  year={2006},
  school={University of Washington}
},
@article{bohte2009deriving,
  title={Deriving and validating trip purposes and travel modes for multi-day {GPS}-based travel surveys: A large-scale application in the {Netherlands}},
  author={Bohte, Wendy and Maat, Kees},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={17},
  number={3},
  pages={285--297},
  year={2009},
  publisher={Elsevier}
},
@article{stopher2008search,
  title={Search for a global positioning system device to measure person travel},
  author={Stopher, Peter and FitzGerald, Camden and Zhang, Jun},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={16},
  number={3},
  pages={350--369},
  year={2008},
  publisher={Elsevier}
},
@article{gong2012gps,
  title={A {GPS/GIS} method for travel mode detection in New York City},
  author={Gong, Hongmian and Chen, Cynthia and Bialostozky, Evan and Lawson, Catherine T},
  journal={Computers, Environment and Urban Systems},
  volume={36},
  number={2},
  pages={131--139},
  year={2012},
  publisher={Elsevier}
},
@article{schuessler2009processing,
  title={Processing raw data from global positioning systems without additional information},
  author={Schuessler, Nadine and Axhausen, Kay W},
  journal={Transportation Research Record: Journal of the Transportation Research Board},
  volume={2105},
  number={1},
  pages={28--36},
  year={2009},
  publisher={Trans Res Board}
},
@inproceedings{hemminki2013accelerometer,
  title={Accelerometer-based transportation mode detection on smartphones},
  author={Hemminki, Samuli and Nurmi, Petteri and Tarkoma, Sasu},
  booktitle={Proceedings of the 11th ACM Conference on Embedded Networked Sensor Systems},
  pages={13},
  year={2013},
  organization={ACM}
},
@article{chang2011libsvm,
  title={LIBSVM: a library for support vector machines},
  author={Chang, Chih-Chung and Lin, Chih-Jen},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={2},
  number={3},
  pages={27},
  year={2011},
  publisher={ACM}
},
@article{figo2010preprocessing,
  title={Preprocessing techniques for context recognition from accelerometer data},
  author={Figo, Davide and Diniz, Pedro C and Ferreira, Diogo R and Cardoso, Jo{\~a}o MP},
  journal={Personal and Ubiquitous Computing},
  volume={14},
  number={7},
  pages={645--662},
  year={2010},
  publisher={Springer}
},
@article{nitsche2012strategy,
  title={A strategy on how to utilize smartphones for automatically reconstructing trips in travel surveys},
  author={Nitsche, Philippe and Widhalm, Peter and Breuss, Simon and Maurer, Peter},
  journal={Procedia-Social and Behavioral Sciences},
  volume={48},
  pages={1033--1046},
  year={2012},
  publisher={Elsevier}
},
@article{feng2013transportation,
  title={Transportation mode recognition using {GPS} and accelerometer data},
  author={Feng, Tao and Timmermans, Harry JP},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={37},
  pages={118--130},
  year={2013},
  publisher={Elsevier}
},
@inproceedings{widhalm2012transport,
  title={Transport mode detection with realistic Smartphone sensor data},
  author={Widhalm, Peter and Nitsche, Philippe and Brandie, N},
  booktitle={Pattern Recognition (ICPR), 2012 21st International Conference on},
  pages={573--576},
  year={2012},
  organization={IEEE}
},
@incollection{lester2006practical,
  title={A practical approach to recognizing physical activities},
  author={Lester, Jonathan and Choudhury, Tanzeem and Borriello, Gaetano},
  booktitle={Pervasive Computing},
  pages={1--16},
  year={2006},
  publisher={Springer}
},
@inproceedings{lu2010jigsaw,
  title={The Jigsaw continuous sensing engine for mobile phone applications},
  author={Lu, Hong and Yang, Jun and Liu, Zhigang and Lane, Nicholas D and Choudhury, Tanzeem and Campbell, Andrew T},
  booktitle={Proceedings of the 8th ACM Conference on Embedded Networked Sensor Systems},
  pages={71--84},
  year={2010},
  organization={ACM}
},@inproceedings{mun2008parsimonious,
  title={Parsimonious mobility classification using GSM and WiFi traces},
  author={Mun, M and Estrin, Deborah and Burke, Jeff and Hansen, Mark},
  booktitle={Proceedings of the Fifth Workshop on Embedded Networked Sensors (HotEmNets)},
  year={2008}
},

@TECHREPORT{anderson2006practical,
  title={Practical Activity Recognition using {GSM} Data},
  author={Anderson, Ian and Muller, Henk},
  year={2006},
  institution =  {Department of Computer Science, University of Bristol},
  number =       {CSTR-06-016},
}

@inproceedings{zheng2008understanding,
  title={Understanding mobility based on {GPS} data},
  author={Zheng, Yu and Li, Quannan and Chen, Yukun and Xie, Xing and Ma, Wei-Ying},
  booktitle={Proceedings of the 10th international conference on Ubiquitous computing},
  pages={312--321},
  year={2008},
  organization={ACM}
},
@inproceedings{miluzzo2008sensing,
  title={Sensing meets mobile social networks: the design, implementation and evaluation of the cenceme application},
  author={Miluzzo, Emiliano and Lane, Nicholas D and Fodor, Krist{\'o}f and Peterson, Ronald and Lu, Hong and Musolesi, Mirco and Eisenman, Shane B and Zheng, Xiao and Campbell, Andrew T},
  booktitle={Proceedings of the 6th ACM conference on Embedded network sensor systems},
  pages={337--350},
  year={2008},
  organization={ACM}
},
@article{yu2014big,
  title={Big Data Small Footprint: The Design of A Low-Power Classifier for Detecting Transportation Modes},
  author={Yu, Meng-Chieh and Yu, Tong and Wang, Shao-Chen and Lin, Chih-Jen and Chang, Edward Y},
  year={2014},
},
@inproceedings{yang2009toward,
  title={Toward physical activity diary: motion recognition using simple acceleration features with mobile phones},
  author={Yang, Jun},
  booktitle={Proceedings of the 1st international workshop on Interactive multimedia for consumer electronics},
  pages={1--10},
  year={2009},
  organization={ACM}
},
@inproceedings{krumm2004locadio,
  title={{LOCADIO}: Inferring Motion and Location from {Wi-Fi} Signal Strengths.},
  author={Krumm, John and Horvitz, Eric},
  booktitle={MobiQuitous},
  pages={4--13},
  year={2004}
},
@incollection{muthukrishnan2007sensing,
  title={Sensing motion using spectral and spatial analysis of WLAN RSSI},
  author={Muthukrishnan, Kavitha and Lijding, Maria and Meratnia, Nirvana and Havinga, Paul},
  booktitle={Smart Sensing and Context},
  pages={62--76},
  year={2007},
  publisher={Springer}
},
@inproceedings{kim2010sensloc,
  title={Sensloc: sensing everyday places and paths using less energy},
  author={Kim, Donnie H and Kim, Younghun and Estrin, Deborah and Srivastava, Mani B},
  booktitle={Proceedings of the 8th ACM Conference on Embedded Networked Sensor Systems},
  pages={43--56},
  year={2010},
  organization={ACM}
},
@inproceedings{kjaergaard2011energy,
  title={Energy-efficient trajectory tracking for mobile devices},
  author={Kj{\ae}rgaard, Mikkel Baun and Bhattacharya, Sourav and Blunck, Henrik and Nurmi, Petteri},
  booktitle={Proceedings of the 9th international conference on Mobile systems, applications, and services},
  pages={307--320},
  year={2011},
  organization={ACM}
},
@article{zheng2010understanding,
  title={Understanding transportation modes based on {GPS} data for web applications},
  author={Zheng, Yu and Chen, Yukun and Li, Quannan and Xie, Xing and Ma, Wei-Ying},
  journal={ACM Transactions on the Web (TWEB)},
  volume={4},
  number={1},
  pages={1},
  year={2010},
  publisher={ACM}
},
@article{bolbol2012inferring,
  title={Inferring hybrid transportation modes from sparse {GPS} data using a moving window {SVM} classification},
  author={Bolbol, Adel and Cheng, Tao and Tsapakis, Ioannis and Haworth, James},
  journal={Computers, Environment and Urban Systems},
  volume={36},
  number={6},
  pages={526--537},
  year={2012},
  publisher={Elsevier}
},
@misc{websitestats2014,
	title = {Global mobile statistics 2014 Part A: Mobile subscribers; handset market share; mobile operators},
	shorttitle = {Global mobile statistics 2014 Part A},
	url = {http://mobithinking.com/mobile-marketing-tools/latest-mobile-stats/asubscribers},
	abstract = {Description:\&nbsp;{MAY} 2014: Put your mobile strategy on a sound footing with The essential mobile stats compendium. Global mobile subscribers (new); top mobile countries (update); handset sales (new), market share (new); smartphone sales (new),},
	urldate = {2014-08-19},
	keywords = {2013, 2014, Android, Apple, handset sales, {HTC}, {iOS}, {LG}, manufacturers, market share, Microsoft, mobile, mobile statistics, mobile subscribers, operating system, phone security, Samsung, smartphone market share, stats, tablets, top mobile countries, top ten, {ZTE}},
},
@misc{webstatandroid,
	title = {Android on 80\% of smart phones shipped in 2013 {\textbar} Canalys},
	url = {http://www.canalys.com/newsroom/android-80-smart-phones-shipped-2013},
	urldate = {2014-08-19},
	file = {Android on 80% of smart phones shipped in 2013 | Canalys:C\:\\Users\\Al_Habib_Al_Mostafa\\AppData\\Roaming\\Zotero\\Zotero\\Profiles\\nkazpk08.default\\zotero\\storage\\UCMMM65C\\android-80-smart-phones-shipped-2013.html:text/html}
},
@misc{webstatandroid2,
	title= {Smartphone {OS} Market Share, {Q2} 2014},
    author= {{International Data Corporation (IDC)}},
	url = {http://www.idc.com/prodserv/smartphone-os-market-share.jsp},
	urldate = {2014-10-10},
}

@article{henderson2008changing,
  title={The changing usage of a mature campus-wide wireless network},
  author={Henderson, Tristan and Kotz, David and Abyzov, Ilya},
  journal={Computer Networks},
  volume={52},
  number={14},
  pages={2690--2712},
  year={2008},
  publisher={Elsevier}
},
@inproceedings{song2004evaluating,
  title={Evaluating location predictors with extensive Wi-Fi mobility data},
  author={Song, Libo and Kotz, David and Jain, Ravi and He, Xiaoning},
  booktitle={INFOCOM 2004. Twenty-third AnnualJoint Conference of the IEEE Computer and Communications Societies},
  volume={2},
  pages={1414--1424},
  year={2004},
  organization={IEEE}
},@inproceedings{yoon2006building,
  title={Building realistic mobility models from coarse-grained traces},
  author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
  booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
  pages={177--190},
  year={2006},
  organization={ACM}
},
@article{yin2008learning,
  title={Learning adaptive temporal radio maps for signal-strength-based location estimation},
  author={Yin, Jie and Yang, Qiang and Ni, Lionel M},
  journal={Mobile Computing, IEEE Transactions on},
  volume={7},
  number={7},
  pages={869--883},
  year={2008},
  publisher={IEEE}
},
@book{rappaport1996wireless,
  title={Wireless communications: principles and practice},
  author={Rappaport, Theodore S and others},
  volume={2},
  year={1996},
  publisher={prentice hall PTR New Jersey}
},
@article{kohavi1997wrappers,
  title={Wrappers for feature subset selection},
  author={Kohavi, Ron and John, George H},
  journal={Artificial intelligence},
  volume={97},
  number={1},
  pages={273--324},
  year={1997},
  publisher={Elsevier}
}

@inproceedings{consolvo2008activity,
  title={Activity sensing in the wild: a field trial of ubifit garden},
  author={Consolvo, Sunny and McDonald, David W and Toscos, Tammy and Chen, Mike Y and Froehlich, Jon and Harrison, Beverly and Klasnja, Predrag and LaMarca, Anthony and LeGrand, Louis and Libby, Ryan and others},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1797--1806},
  year={2008},
  organization={ACM}
}

@inproceedings{snapnet,
  title={Accurate and Efficient Map Matching for Challenging Environments},
  author={Reham Mohamed and Heba Aly and Moustafa Youssef},
  booktitle={Proceedings of the 22nd ACM SIGSPATIAL International Conference on Advances in Geographic Information Systems},
  year={2014},
  organization={ACM}
}

@inproceedings{mohan2008nericell,
  title={Nericell: rich monitoring of road and traffic conditions using mobile smartphones},
  author={Mohan, Prashanth and Padmanabhan, Venkata N and Ramjee, Ramachandran},
  booktitle={Proceedings of the 6th ACM conference on Embedded network sensor systems},
  pages={323--336},
  year={2008},
  organization={ACM}
}

@misc{wiki_api,
author = "Wikipedia",
   title = "Android version history --- Wikipedia{,} The Free Encyclopedia",
   year = "2014",
   url = "http://en.wikipedia.org/w/index.php?title=Android_version_history&oldid=599583037",
   note = "[Online; accessed 1-March-2014]"
}

@inproceedings{ibrahim2011hidden,
  title={A hidden markov model for localization using low-end {GSM} cell phones},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  booktitle={ICC},
  year={2011},
  organization={IEEE}
}
@article{cellsense,
  title={Cell{S}ense: {A}n accurate energy-efficient {GSM} positioning system},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  journal={IEEE TVT},
  year={2012},
  publisher={IEEE}
}
@inproceedings{ibrahim2010cellsense,
  title={Cell{S}ense: {A} probabilistic {RSSI}-based {GSM} positioning system},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  booktitle={GLOBECOM},
  year={2010},
  organization={IEEE}
}
@inproceedings{ibrahim2013enabling,
  title={Enabling wide deployment of {GSM} localization over heterogeneous phones},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  booktitle={ICC},
  year={2013},
  organization={IEEE}
}

@inproceedings{aly2013dejavu,
  title={Dejavu: an accurate energy-efficient outdoor localization system},
  author={Aly, Heba and Youssef, Moustafa},
  booktitle={SIGSPATIAL GIS},
  year={2013},
  organization={ACM}
}

@inproceedings{sheikh2014demonstrating,
  title={Demonstrating {M}ap++: {A} crowd-sensing system for automatic map semantics identification},
  author={Sheikh, Shuja Jamil and Basalamah, Anas and Aly, Heba and Youssef, Moustafa},
  booktitle={SECON},
  year={2014},
  organization={IEEE}
}
@inproceedings{mohssen2014s,
  title={It's the human that matters: {A}ccurate user orientation estimation for mobile computing applications},
  author={Mohssen, Nesma and Momtaz, Rana and Aly, Heba and Youssef, Moustafa},
  booktitle={MobiQuitous},
  year={2014},
  organization={ICST}
}
@inproceedings{GAC,
  title={{GAC}: energy-efficient hybrid {GPS}-accelerometer-compass {GSM} localization},
  author={Youssef, Moustafa and Yosef, M Amir and El-Derini, Mohamed},
  booktitle={GLOBECOM},
  year={2010},
  organization={IEEE}
}

@inproceedings{aly_map14,
title={Map++: {A} crowd-sensing system for automatic map semantics identification},
author={Aly, Heba and Basalamah, Anas and Youssef, Moustafa},
  booktitle={SECON},
  year={2014},
  organization={IEEE}
}

@inproceedings{al2012rf,
	Author = {Al-Husseiny, Amal and Youssef, Moustafa},
	Booktitle = {IEEE Vehicular Technology Conference (VTC Fall), 2012},
	Title = {{RF}-based Traffic Detection and Identification},
	Year = {2012}}
	
@inproceedings{Kassem:VTC12,
  	author = {Nehal Kassem and Ahmed E. Kosba and Moustafa Youssef},
  	title = {{RF}-based Vehicle Detection and Speed Estimation},
 	booktitle = {IEEE VTC Spring},
  	year = {2012},
}

